SSUL: Semantic Segmentation with Unknown Label for Exemplar-based Class-Incremental Learning

This paper introduces a solid state-of-the-art baseline for a class-incremental semantic segmentation (CISS) problem. While the recent CISS algorithms utilize variants of the knowledge distillation (KD) technique to tackle the problem, they failed to fully address the critical challenges in CISS causing the catastrophic forgetting; the semantic drift of the background class and the multi-label prediction issue. To better address these challenges, we propose a new method, dubbed SSUL-M (Semantic Segmentation with Unknown Label with Memory), by carefully combining techniques tailored for semantic segmentation. Specifically, we claim three main contributions. (1) defining unknown classes within the background class to help to learn future classes (help plasticity), (2) freezing backbone network and past classifiers with binary cross-entropy loss and pseudo-labeling to overcome catastrophic forgetting (help stability), and (3) utilizing tiny exemplar memory for the first time in CISS to improve both plasticity and stability. The extensively conducted experiments show the effectiveness of our method, achieving significantly better performance than the recent state-of-the-art baselines on the standard benchmark datasets. Furthermore, we justify our contributions with thorough ablation analyses and discuss different natures of the CISS problem compared to the traditional class-incremental learning targeting classification. The official code is available at https://github.com/clovaai/SSUL.

==> Experiments__deprecated_.tex <==
% % \clearpage


% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%     \begin{adjustbox}{max width=\linewidth}
%       \begin{tabular}{c|cccccc|ccc|ccc}
%         \hline
%             & & &        &     &        &        & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} & \multicolumn{3}{|c}{\textbf{10-1 (11 tasks)}} \\
%         exp & PL & unknown & transfer & freeze & sigmoid & memory & 0-15 & 16-20 & all & 1-11 & 11-20 & all \\
%         \hline
%         \hline
%         1 & &           &        &  &  &        & 04.32 & 02.36 & 03.86 &  0   &   0   &  0  \\
%         2 & &           &        & \checkmark &  &        & 04.33 & 12.35 & 06.24 &  0   &   0   &  0  \\
%         3 & \checkmark &  &  &     &        &        & 16.73 & 08.43 & 14.76 &  0   &   0   &  0  \\
%         4 & \checkmark &  &  & \checkmark &        &        & 43.96 & 16.85 & 37.51 &  0   &   0   &  0  \\
%         \hline
%         5 & &           &        &     & \checkmark &        & 04.31 & 02.25 & 03.82 &  0   &   0   &  0  \\
%         6 & &           &        & \checkmark & \checkmark &        & 47.43 & 12.70 & 39.16 &  0   &   0   &  0  \\
%         7 & \checkmark &  &  &     & \checkmark &        & 28.12 & 12.23 & 24.34 &  0   &   0   &  0  \\
%         %\checkmark &  &  & \checkmark & \checkmark &        & 78.15 & 11.27 & 62.23 &  0   &   0   &  0  \\
%         8 & \checkmark &  &  & \checkmark & \checkmark &        & 73.42 & 21.79 & 61.12 &  0   &   0   &  0  \\
%         \hline
%         9 & \checkmark & \checkmark &  &     &        &        & 23.55 & 05.60 & 19.27 & 0 & 0 & 0     \\
%         10 & \checkmark & \checkmark & \checkmark &     &        &        & 52.15 & 21.82 & 44.92 & 0 & 0 & 0     \\
%         11 & \checkmark & \checkmark &  & \checkmark &        &        & 53.99 & 21.84 & 46.33 & 0 & 0 & 0     \\
%         12 & \checkmark & \checkmark & \checkmark & \checkmark &        &        & 53.02 & 21.62 & 45.54 & 0 & 0 & 0     \\
%         13 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &        & 78.06 & 28.54 & 66.27 & 73.78 & 41.13 & 58.23  \\
%         14 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 78.92 & 43.86 & 70.58 & 74.79 & 48.87 & 62.45  \\
%          \hline
%          15 & \checkmark & \checkmark & \checkmark &  & \checkmark &  & 53.56 & 14.48 & 44.25 & 0 & 0 & 0 \\
%          16 & \checkmark & \checkmark &  & \checkmark & \checkmark &  & 73.73 & 23.99 & 61.89 & 0 & 0 & 0  \\
%          17 & \checkmark & \checkmark &  &  & \checkmark &  & 43.12 & 06.09 & 34.30 & 0 & 0 & 0 \\
%          %18 & & \checkmark & \checkmark & \checkmark & \checkmark &  & \by{76.78} & \by{31.71} & \by{66.05} & 0 & 0 & 0  \\
         
%         \hline
%       \end{tabular}
%     \end{adjustbox}
%   \caption{
%     Ablation study on PASCAL VOC 2012 dataset. PL (pseudo labeling); unknown (unknown label using saliency maps); freeze (network freezing); sigmoid (change from softmax-CE-loss to sigmoid-CE-loss; memory (replay 100 labels); cutmix (applying cutmix algorithm between current labels and memory labels)
%   }
%   \label{tab:ablation}
% \end{table}
% %------------------------------------------------------------------------------------



% %--------------------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     Experimental results on ADE20K. SSUL$\dagger$ denotes the result using exemplar memory.
%   }
%   \label{tab:sota_ade}
%   \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{c||ccc|ccc|ccc|ccc}
%     \toprule
%      &  \multicolumn{3}{|c}{\textbf{ADE 100-5 (11 tasks)}} & \multicolumn{3}{|c}{\textbf{ADE 100-10 (6 tasks)}} & \multicolumn{3}{|c}{\textbf{ADE 50-50 (3 tasks)}} & \multicolumn{3}{|c}{\textbf{ADE 100-50 (2 tasks)}}  \\
%     Method & 0-100 & 101-150 & all & 0-100 & 101-150 & all & 0-50 & 51-150 & all & 0-100 & 101-150 & all \\
%     \hline
%     ILT \cite{(ILT)michieli2019incremental} & 0.08 & 1.31 & 0.49 & 0.11 & 3.06 & 1.09 & 3.53 & 12.85 & 9.70 & 18.29 & 14.40 & 17.00 \\
%     MiB \cite{(MiB)cermelli2020modeling} & 36.01 & 5.66 & 25.96 & 38.21 & 11.12 & 29.24 & 45.57 & 21.01 & 29.31 & 40.52 & 17.17 & 32.79 \\
%     PLOP \cite{(PLOP)douillard2020plop} & 39.11 & 7.81 & 28.75 & 40.48 & 13.61 & 31.59 & 48.83 & 20.99 & 30.40 & 41.87 & 14.89 & 32.94 \\
%     \hline
%     SSUL & 42.03 & 15.80 & 33.35 & 42.10 & 16.02 & 33.46 & - & - & - & 42.12 & 12.76 & 32.40  \\
%     SSUL$\dagger$ & - & - & - & - & - & - & - & - & -  & - & - & - \\
%     %\hline
%     %Joint & 44.30 & 28.20 & 38.90 & 44.30 & 28.20 & 38.90 & 51.10 & 33.25 & 38.90 & 51.10 & 33.25 & 38.90 & 44.30 & 28.20 & 38.90  \\
%     \bottomrule
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{-2mm}
% \end{table}
% %--------------------------------------------------------------------------------------------------



% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     Ablation study : class ordering.
%   }
% \label{tab:sota_maskrcnn}

% \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{c|cccccccccccccccccccc|cc}
%     \hline
%     \textbf{15-1 (6 tasks)} & \multicolumn{20}{|c|}{\textbf{Class Ordering}} & \textbf{min} & \textbf{max}\\
%      & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 &  &  \\
%     \hline
%     %1-15  & 77.94 & 78.56 & 78.54 & 78.62 & 78.56 & 78.56 & 78.51 & 78.49 & 78.51 & 78.61 \\ 
%     %16-20 & 27.76 & 30.65 & 32.18 & 34.57 & 36.00 & 34.62 & 34.10 & 34.43 & 34.65 & 36.51 \\
%     %all   & 66.00 & 67.15 & 67.50 & 68.13 & 68.43 & 68.10 & 67.93 & 68.00 & 68.07 & 68.58 \\
%     %\hline
%     %1-15  & 77.94 & 78.79 &       & 78.73 &       & 78.63 &       & 78.58 &       & 78.69 \\ 
%     %16-20 & 27.76 & 38.78 &       & 37.84 &       & 37.30 &       & 37.49 &       & 38.79 \\
%     %all   & 66.00 & 69.26 &       & 68.99 &       & 68.79 &       & 68.79 &       & 69.19 \\
%     %\hline
%     1-15  & 78.06 & 74.46 & 73.32 & 75.45 & 77.43 & 71.72 & 76.56 & 81.50 & 75.06 & 74.19 & 76.94 & 80.30 & 78.69 & 78.30 & 72.72 & 77.65 & 74.83 & 75.29 & 74.71 & 74.11 & 71.72 & 81.50\\ 
%     16-20 & 28.54 & 29.25 & 23.48 & 38.03 & 34.54 & 32.83 & 18.97 & 20.23 & 36.35 & 23.02 & 30.50 & 35.21 & 40.31 & 15.88 & 37.26 & 27.44 & 26.35 & 27.25 & 46.56 & 50.66 & 15.88 & 50.66 \\ 
%     all   & 66.27 & 63.70 & 61.45 & 66.54 & 67.22 & 62.46 & 62.85 & 66.91 & 65.84 & 62.00 & 65.88 & 69.57 & 69.55 & 63.44 & 64.28 & 65.70 & 63.29 & 63.85 & 68.00 & 68.53 & 61.45 & 69.57\\ 
%     \hline
%     1-15  & 78.92 & 75.25 & 74.25 & 76.82 & 78.39 & 72.89 & 77.25 & 81.99 & 75.59 & 74.25 & 77.31 & 80.07 & 78.56 & 78.73 & 75.30 & 78.25 & 76.27 & 75.49 & 74.59 & 74.17 \\
%     16-20 & 43.86 & 46.26 & 54.53 & 61.88 & 51.93 & 60.00 & 39.09 & 36.11 & 54.23 & 54.08 & 44.70 & 43.90 & 48.91 & 38.27 & 52.98 & 44.28 & 55.42 & 52.62 & 51.23 & 58.45 \\
%     all   & 70.58 & 68.35 & 69.55 & 73.27 & 72.09 & 69.82 & 68.16 & 71.06 & 70.51 & 69.43 & 69.55 & 71.46 & 71.50 & 69.10 & 69.98 & 70.17 & 71.30 & 70.05 & 69.03 & 70.42 \\
%     \hline
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{5mm}

% \end{table}
% %------------------------------------------------------------------------------------



% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     Ablation study: memory sampling (memory 100)
%   }
% \label{tab:sota_maskrcnn}

% \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{cc|cc|ccc|ccc}
%     \hline
%      & & \multicolumn{2}{|c}{(deprecated)} & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} & \multicolumn{3}{|c}{\textbf{10-1 (11 tasks)}} \\
%     class-balanced & pseudo-label & priority & cutmix & 1-15 & 16-20 & all & 1-11 & 11-20 & all \\
%     \hline
%     &  &  &  & 78.61 & 38.87 & 69.15 \\
%     & \checkmark &  &  & 78.55 & 38.36 & 68.98 \\
%     \checkmark &  &  &  & 78.92 & 43.86 & 70.58 & 74.79 & 48.87 & 62.45 \\
%     \checkmark & \checkmark (0.5) &  &  & 78.92 & 42.86 & 70.34 & 74.87 & 47.58 & 61.87\\
%     \checkmark & \checkmark (0.8) &  &  & 78.94 & 43.97 & 70.61 & 74.76 & 48.21 & 62.11 \\
%     \hline
%     %\checkmark &  & \checkmark &  & 78.60 & 38.28 & 69.00 \\
%      & \checkmark & \checkmark &  & 78.59 & 38.38 & 69.01 \\
%     \checkmark & \checkmark & \checkmark &  & 78.88 & 40.82 & 69.82 & 74.72 & 47.30 & 61.66 \\
%     \checkmark & \checkmark & \checkmark & \checkmark & 78.71 & 33.53 & 67.95 \\
%     \hline
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{5mm}

% \end{table}
% %------------------------------------------------------------------------------------



% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     SOTA comparison. mem: memory 100.
%   }
% \label{tab:sota_maskrcnn}

% \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{c|cccc|cccc|cccc}
%     \hline
%      &  \multicolumn{4}{|c}{\textbf{10-1 (11 tasks)}} & \multicolumn{4}{|c}{\textbf{5-5 (4 tasks)}} & \multicolumn{4}{c}{\textbf{5-3 (6 tasks)}}   \\
%     Method & 1-10 & 11-20 & all & exp & 1-5 & 5-20 & all & exp & 1-5 & 5-20 & all & exp  \\
%     \hline
%     ILT & 07.15 & 03.67 & 05.50 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
%     MiB & 12.25 & 13.09 & 12.65 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%     PLOP & 44.03 & 15.51 & 30.45 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%     \hline
%     ILT (rep) & 07.17 & 03.21 & 05.29 & (K1579) & 47.28 & 41.17 & 42.92 & (K1560) & 22.51 & 31.66 & 29.04 & (K1561) \\
%     MiB (rep) & 12.29 & 14.65 & 13.41 & (K1578) & 71.10 & \textbf{55.17} & \textbf{59.72} & (K1558) & 57.10 & 42.56 & 46.71 & (K1559) \\
%     PLOP (rep) & 27.13 & 15.51 & 21.60 & (K1577) & 34.77 & 20.77 & 24.77 & (b1411) & 17.48 & 19.16 & 18.68 & (K1533) \\
%     \hline
%     ours & \textbf{73.78} & \textbf{41.13} & \textbf{58.23} & (b1241) & \textbf{72.42} & 46.79 & 54.11 & (b1242) & \textbf{71.17} & \textbf{45.38} & \textbf{52.75} & (b1348) \\
%     ours + mem & \textbf{74.72} & \textbf{47.30} & \textbf{61.66} & (b1398) & \textbf{72.30} & 50.41 & 56.66 & (b1401) & \textbf{73.09} & \textbf{47.56} & \textbf{54.85} & (b1403) \\
    
%     %ours & 73.27 & 40.14 & 57.49 & (b1051) & 72.25 & 46.55 & 53.90 & (b1127) & 70.57 & 44.76 & 52.14 & (b1196) \\
%     %ours + thresh & 73.78 & 41.13 & 58.23 & (b1241) & 72.42 & 46.79 & 54.11 & (b1242) & 71.17 & 45.38 & 52.75 & (b1348) \\
%     %ours + mem & 74.23 & 47.21 & 61.36 & (b1148) & 72.30 & 49.77 & 56.21 & (b1344) & 72.91 & 49.02 & 55.85 & (b1354) \\
%     %ours + mem2 & 74.72 & 47.30 & 61.66 & (b1398) & 72.30 & 50.41 & 56.66 & (b1401) & 73.09 & 47.56 & 54.85 & (b1403) \\
%     \hline
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{5mm}

% \end{table}
% %------------------------------------------------------------------------------------



% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     SOTA comparison. mem: memory 100.
%   }
% \label{tab:sota_maskrcnn}

% \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{c|cccc|cccc|cccc}
%     \hline
%      &  \multicolumn{4}{|c}{\textbf{15-1 (6 tasks)}} & \multicolumn{4}{c}{\textbf{15-5 (2 tasks)}} & \multicolumn{4}{|c}{\textbf{19-1 (2 tasks)}}  \\
%     Method & 1-15 & 16-20 & all & exp & 1-15 & 16-20 & all & exp & 1-19 & 20 & all & exp  \\
%     \hline
%     ILT & 8.75 & 7.99 & 8.56 & & 67.08 & 39.23 & 60.45 & &  67.75 & 10.88 & 65.05  \\
%     MiB & 34.22 & 13.50 & 29.29 & & 76.37 & 49.97 & 70.08 & &  71.43 & 23.59 & 69.15 \\
%     PLOP & 65.12 & 21.11 & 54.64 & & 75.73 & \textbf{51.71} & 70.09 & &  75.35 & \textbf{37.35} & 73.54  \\
%     \hline
%     ours & \textbf{77.94} & \textbf{27.76} & \textbf{66.00} & (1032) & \textbf{78.00} & 46.74 & \textbf{70.56} & (1083) &  \textbf{78.44} & 26.02 & \textbf{75.94} & (1041)  \\
%     ours + thresh & 78.06 & 28.54 & 66.27 & (1234) & 77.88 & 46.08 & 70.31 & (1239) & 78.52 & 27.23 & 76.07 & (1240)  \\
%     ours + mem & 78.88 & 40.82 & 69.82 & (1329) & \textbf{79.44} & \textbf{51.76} & \textbf{72.85} & (1146) & \textbf{78.47} & 36.11 & \textbf{76.45} & (1336) \\
%     ours + mem2 & 78.92 & 42.86 & 70.34 & (1379) & 79.44 & 52.27 & 72.97 & (1393) & 78.52 & 40.12 & 76.69 & (1400) \\
%     ours + mem3 & 78.92 & 43.86 & 70.58 & (1406) & 0 & 0 & 0 & (0) & 0 & 0 & 0 & (0) \\
%     \hline
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{5mm}

% \end{table}
% %------------------------------------------------------------------------------------







% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     SOTA comparison. mem: memory 100.
%   }
% \label{tab:sota_maskrcnn}

% \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{c|ccc|ccc|ccc}
%     \hline
%      &  \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} & \multicolumn{3}{c}{\textbf{15-5 (2 tasks)}} & \multicolumn{3}{|c}{\textbf{19-1 (2 tasks)}}  \\
%     Method & 1-15 & 16-20 & all & 1-15 & 16-20 & all & 1-19 & 20 & all  \\
%     \hline
%     EWC  & 0.30 & 4.30 & 1.30 & 24.30 & 35.50 & 27.10  & 26.90 & 14.00 & 26.30 \\
%     LwF-MC & 6.40 & 8.40 & 6.90 & 58.10 & 35.00 & 52.30  & 64.40 & 13.30 & 61.90   \\
%     ILT & 8.75 & 7.99 & 8.56 & 67.08 & 39.23 & 60.45 &  67.75 & 10.88 & 65.05  \\
%     MiB & 34.22 & 13.50 & 29.29 & 76.37 & 49.97 & 70.08 &  71.43 & 23.59 & 69.15 \\
%     PLOP & 65.12 & 21.11 & 54.64 & 75.73 & \textbf{51.71} & 70.09 &  75.35 & \textbf{37.35} & 73.54  \\
%     %self-training & 76.70 & 54.30 & 71.10 & 71.40 & 40.00 & 63.60 & 76.10 & 43.40 & 74.50 \\
%     \hline
%     %PLOP$\dagger$ & 74.97 & 49.91 & 69.01 & 66.51 & 21.20 & 55.72 & 75.23 & 34.27 & 73.28 \\
%     %PLOP$\dagger$ (sigmoid) & 67.63 & 34.21 & 59.67 & 47.32 & 11.43 & 38.77 & 76.90 & 30.79 & 74.70 \\
%     %\hline
%     %ours  & 74.90 & 15.71 & \textbf{60.81} & 77.42 & 47.16 & \textbf{70.21} &  77.09 & 28.69 & \textbf{74.78} \\
%     ours & \textbf{78.06} & \textbf{28.54} & \textbf{66.27} & \textbf{78.00} & 46.74 & \textbf{70.56} & \textbf{78.52} & 27.23 & \textbf{76.07}   \\
%     ours$\dagger$ &  \textbf{78.92} & \textbf{43.86} & \textbf{70.58} & \textbf{79.53} & \textbf{52.87} & \textbf{73.19} & \textbf{78.52} & \textbf{40.51} & \textbf{76.71} \\
%     %ours + mem 100 & \textbf{78.77} & \textbf{47.00} & \textbf{71.20}  & \textbf{77.99} & \textbf{38.82} & \textbf{68.67} & \textbf{76.85} & \textbf{40.42} & \textbf{75.12} \\
%     %ours + mem 100 + cutmix & 78.25 & 47.29 & 70.85 & 77.29 & 31.28 & 66.39 & 75.89 & 24.48 & 73.32 \\
%     \hline
%     Joint & 79.10 & 72.60 & 77.40 & 79.10 & 72.60 & 77.40  & 79.10 & 72.60 & 77.40  \\
%     \hline
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{5mm}

% \end{table}
% %------------------------------------------------------------------------------------

% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     PASCAL VOC 2012 with 15-5 case. PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map); Fix (fixed prev network); Stack;
%   }
% \label{tab:sota_maskrcnn}

% \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{c|ccc|ccc|ccc}
%     \hline
%      & \multicolumn{3}{|c}{\textbf{10-1 (11 tasks)}} & \multicolumn{3}{|c}{\textbf{5-5 (4 tasks)}} & \multicolumn{3}{c}{\textbf{5-3 (6 tasks)}}  \\
%     Method & 1-10 & 11-20 & all & 1-5 & 5-20 & all & 1-5 & 5-20 & all   \\
%     \hline
%     ILT  & 7.15 & 3.67 & 5.50 & 47.28 & 41.17 & 42.92 & 22.51 & 31.66 & 29.04   \\
%     MiB  & 12.25 & 13.09 & 12.65 & 71.10 & 55.17 & 59.72 & 57.10 & 42.56 & 46.71    \\
%     PLOP & 44.03 & 15.51 & 30.45 & 34.77 & 20.76 & 24.77 & 17.48 & 19.16 & 18.68    \\
%     %self-training & 76.70 & 54.30 & 71.10 & 71.40 & 40.00 & 63.60 & 76.10 & 43.40 & 74.50 \\
%     \hline
%     %PLOP$\dagger$ & 74.97 & 49.91 & 69.01 & 66.51 & 21.20 & 55.72 & 75.23 & 34.27 & 73.28 \\
%     %PLOP$\dagger$ (sigmoid) & 67.63 & 34.21 & 59.67 & 47.32 & 11.43 & 38.77 & 76.90 & 30.79 & 74.70 \\
%     %\hline
%     ours  & \textbf{73.78} & \textbf{41.13} & \textbf{58.23} & \textbf{72.42} & \textbf{46.79} & \textbf{54.11} & 71.17 & 45.38 & 52.75  \\
%     ours$\dagger$ & \textbf{74.79} & \textbf{48.87} & \textbf{62.45} & 72.34 & 50.23 & 56.55 & 72.91 & 49.02 & 55.85 \\
%     \hline
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{5mm}

% \end{table}
% %------------------------------------------------------------------------------------


% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     Ablation study : the effect of memory size.
%   }
% \label{tab:sota_maskrcnn}

% \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{c|ccccccccccccc}
%     \hline
%     \textbf{15-1 (6 tasks)} & \multicolumn{10}{|c}{\textbf{Memory Size}} \\
%      & 0 & 20 & 40 & 60 & 80 & 100 & 120 & 140 & 160 & 180 & 200 & 300 & 400 \\
%     \hline
%     %1-15  & 77.94 & 78.56 & 78.54 & 78.62 & 78.56 & 78.56 & 78.51 & 78.49 & 78.51 & 78.61 \\ 
%     %16-20 & 27.76 & 30.65 & 32.18 & 34.57 & 36.00 & 34.62 & 34.10 & 34.43 & 34.65 & 36.51 \\
%     %all   & 66.00 & 67.15 & 67.50 & 68.13 & 68.43 & 68.10 & 67.93 & 68.00 & 68.07 & 68.58 \\
%     %\hline
%     %1-15  & 77.94 & 78.79 &       & 78.73 &       & 78.63 &       & 78.58 &       & 78.69 \\ 
%     %16-20 & 27.76 & 38.78 &       & 37.84 &       & 37.30 &       & 37.49 &       & 38.79 \\
%     %all   & 66.00 & 69.26 &       & 68.99 &       & 68.79 &       & 68.79 &       & 69.19 \\
%     %\hline
%     % 1-15  & 77.94 & 78.77 & 78.79 & 78.91 & 78.88 & 78.86 & 78.92 & 78.83 & 78.87 & 78.90 & 78.95 & 79.03 \\ 
%     % 16-20 & 27.76 & 38.62 & 39.97 & 39.07 & 40.82 & 39.62 & 40.41 & 39.35 & 39.36 & 40.89 & 41.11 & 41.19 \\ 
%     % all   & 66.00 & 69.21 & 69.55 & 69.42 & 69.82 & 69.52 & 69.75 & 69.43 & 69.46 & 69.85 & 69.94 & 70.02 \\ 
%     % \hline
%     1-15  & 78.06 & 78.74 & 78.86 & 78.93 & 78.80 & 78.92 & 79.06 & 78.98 & 79.09 & 79.04 & 79.02 & 79.02 & 79.08 \\
%     16-20 & 28.54 & 41.00 & 41.08 & 42.44 & 42.35 & 43.86 & 44.03 & 43.32 & 44.04 & 44.04 & 44.22 & 43.37 & 44.89 \\
%     all   & 66.27 & 69.75 & 69.86 & 70.24 & 70.12 & 70.58 & 70.72 & 70.49 & 70.74 & 70.70 & 70.73 & 70.54 & 70.94 \\
%     \hline
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{5mm}

% \end{table}
% %------------------------------------------------------------------------------------






% % %------------------------------------------------------------------------------------
% % \begin{table}[t]
% %   \centering
% %   \caption{
% %     PLOP with our proposed components.
% %   }
% % \label{tab:sota_maskrcnn}

% % \begin{adjustbox}{max width=\linewidth}
% %   \begin{tabular}{c|ccc}
% %     \hline
% %       & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} \\
% %     Method & 1-15 & 16-20 & all \\
% %     \hline
% %     PLOP & 65.12 & 21.11 & 54.64 \\
% %     PLOP + unknown & - & - & - \\
% %     PLOP + unknown + sigmoid & - & - & - \\
% %     PLOP + unknown + sigmoid + memory & - & - & - \\
% %     \hline
% %   \end{tabular}
% %   \end{adjustbox}
% %   \vspace{5mm}

% % \end{table}
% % %------------------------------------------------------------------------------------



% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     Hyperparameter Settings.
%   }
% \label{tab:sota_maskrcnn}

% \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{c|cccccc}
%     \hline
%       & \textbf{10-1 (11 tasks)} & \textbf{15-1 (6 tasks)} & \textbf{15-5 (2 tasks)} & \textbf{19-1 (2 tasks)} & \textbf{5-5 (4 tasks)} & \textbf{5-3 (6 tasks)}\\
%     \hline
%     $lr$     & 1e-2 & 1e-2 & 1e-2 & 1e-2 & 1e-2 & 1e-2 \\
%     $lr_{u}$ & 1e-2 & 1e-2 & 1e-2 & 1e-2 & 1e-2 & 1e-2 \\
%     $lr_{b}$ & 1e-5 & 1e-5 & 1e-6 & 1e-5 & 1e-5 & 1e-5 \\
%     BN       & freeze & freeze & freeze & freeze & freeze & freeze \\
%     \hline
%     iter     & 500 & 500 & 5000 & 4000 & 5000 & 5000 \\
%     warm-up   & 50  & 0 & 0  & 200  & 0   & 50    \\
%     \hline
%     session  & backbone/1051 & backbone/1032 & backbone/1083 & backbone/1041 & backbone/1127 & backbone/1196 \\
%     PL thresh & backbone/1241 & backbone/1234 & backbone/1239 & backbone/1240 & backbone/1242 & backbone/1348  \\
%     memory   & backbone/1338 & backbone/1329 & backbone/1334 & backbone/1336 & backbone/1344 & backbone/1354  \\
%     memory2   & backbone/1398 & backbone/1379 & backbone/1393 & backbone/1400 & backbone/1401 & backbone/1403  \\
%     memory3   & backbone/1563 & backbone/1406 & backbone/1598 & backbone/1599 & backbone/1600 & backbone/1602  \\
    
%     \hline
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{5mm}

% \end{table}
% %------------------------------------------------------------------------------------








% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     Ablation study : weight transfer of new head
%   }
% \label{tab:sota_maskrcnn}

% \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{c|ccc}
%     \hline
%     weight  & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} \\
%             & 1-15 & 16-20 & all \\
%     \hline
%     random & 73.73 & 23.99 & 61.89 \\
%     w.background & 73.29 & 23.70 & 61.48 \\
%     w.unknown & \textbf{77.94} & \textbf{27.76} & \textbf{66.00} \\
%     \hline
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{5mm}

% \end{table}
% %------------------------------------------------------------------------------------



% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \caption{
%     Ablation study : saliency map dependency check.
%   }
% \label{tab:sota_maskrcnn}

% \begin{adjustbox}{max width=\linewidth}
%   \begin{tabular}{c|ccc}
%     \hline
%       & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} \\
%     sal map & 1-15 & 16-20 & all \\
%     \hline
%     DRFI (ML-based)  & - & - & - \\
%     DSS (DL-based) & 78.06 & 28.54 & 66.27 \\
%     ground-truth & 79.15 & 29.01 & 67.21 \\
%     \hline
%   \end{tabular}
%   \end{adjustbox}
%   \vspace{5mm}

% \end{table}
% %------------------------------------------------------------------------------------







% % \begin{table}[t]
% % \begin{minipage}[t]{0.5\textwidth}
% %   \centering
% %     \begin{adjustbox}{max width=\linewidth}
% %         \includegraphics{cvpr2021/figures/class_ordering.png}
% %     \end{adjustbox}
% %     \captionof{figure}{Robustness to class ordering}
% %     \label{fig:class_ordering}
% % \end{minipage} \hfill
% % \begin{minipage}[t]{0.5\textwidth}
% %   \centering
% %     \begin{adjustbox}{max width=\linewidth}
% %         \includegraphics{cvpr2021/figures/evolution.png}
% %     \end{adjustbox}
% %     \captionof{figure}{mIoU evolution on Pascal VOC 2012}
% %     \label{fig:miou_evolution}
% % \end{minipage}
% % \end{table}

% \begin{table}[t]
% \begin{minipage}[b]{0.56\textwidth}
%   \centering
%     \begin{adjustbox}{max width=\linewidth}
%         \includegraphics{cvpr2021/figures/memory_size.png}
%     \end{adjustbox}
%     \captionof{figure}{memory size}
%     \label{fig:memory_size}
% \end{minipage} \hfill
% \begin{minipage}[b]{0.44\textwidth}
%   \centering
%   \begin{adjustbox}{max width=\linewidth}
%      \begin{tabular}{c|ccc}
%       \hline
%         & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} \\
%         sal map & 0-15 & 16-20 & all \\
%         \hline
%         wo unknown & 73.42 & 21.79 & 61.12 \\
%         DRFI (ML-based)  & 77.46 & 27.21 & 65.63 \\
%         DSS (DL-based) & 78.06 & 28.54 & 66.27 \\
%         ground-truth & 79.15 & 29.01 & 67.21 \\
%         \hline
%     \end{tabular}
%   \end{adjustbox}
%   \captionof{table}{Dependency on saliency map}
%   \label{tab:salmap_dependency}
%   \vspace{4mm}
%   \begin{adjustbox}{max width=\linewidth}
%      \begin{tabular}{c|ccc}
%       \hline
%           & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} \\
%         weight init  & 0-15 & 16-20 & all \\
%         \hline
%         random & 73.73 & 23.99 & 61.89 \\
%         w.background & 73.29 & 23.70 & 61.48 \\
%         w.unknown & \textbf{77.94} & \textbf{27.76} & \textbf{66.00} \\
%         \hline
%     \end{tabular}
%   \end{adjustbox}
%   \captionof{table}{Effect of knowledge transfer}
%   \label{tab:knowledge_transfer}
% \end{minipage}
% \end{table}



% %------------------------------------------------------------------------------------
% \begin{table}[t]
%   \centering
%   \begin{adjustbox}{max width=\linewidth}
%     \begin{tabular}{c|ccc}
%       \hline
%              & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} \\
%              & 0-15 & 16-20 & all \\
%       \hline
%       \hline
%       \multicolumn{4}{c}{\textbf{Saliency map}} \\
%       -               & 73.42 & 21.79 & 61.12 \\
%       DRFI (ML-based) & 77.46 & 27.21 & 65.63 \\
%       DSS (DL-based)  & 78.06 & 28.54 & 66.27 \\
%       ground-truth    & 79.15 & 29.01 & 67.21 \\
%       \hline
%       \hline
%       \multicolumn{4}{c}{\textbf{Weight Initialize}} \\
%       random & 73.73 & 23.99 & 61.89 \\
%       w.background & 73.29 & 23.70 & 61.48 \\
%       w.unknown & \textbf{77.94} & \textbf{27.76} & \textbf{66.00} \\
%       \hline
%       \hline
%       \multicolumn{4}{c}{\textbf{Memory Sampling}} \\
%       random & 78.61 & 38.87 & 69.15 \\
%       balanced & 78.92 & 43.86 & 70.58 \\
%       \hline
%     \end{tabular}
%   \end{adjustbox}
%   \caption{
%     Ablation study: memory sampling (memory 100)
%   }
% \label{tab:mem_sampling}
% \end{table}
% %------



% \begin{table}[t]
% \begin{minipage}[t]{0.5\textwidth}
%       \begin{table}[t]
%         \centering
%         \caption{
%           Experimental results on ADE20K. SSUL$\dagger$ denotes the result using exemplar memory.
%         }
%         \label{tab:sota_ade}
%         \begin{adjustbox}{max width=\linewidth}
%         \begin{tabular}{c||ccc|ccc}
%           \toprule
%           &  \multicolumn{3}{|c}{\textbf{ADE 100-5 (11 tasks)}} & \multicolumn{3}{|c}{\textbf{ADE 100-10 (6 tasks)}}  \\
%           Method & 0-100 & 101-150 & all & 0-100 & 101-150 & all  \\
%           \hline
%           ILT \cite{(ILT)michieli2019incremental} & 0.08 & 1.31 & 0.49 & 0.11 & 3.06 & 1.09  \\
%           MiB \cite{(MiB)cermelli2020modeling} & 36.01 & 5.66 & 25.96 & 38.21 & 11.12 & 29.24  \\
%           PLOP \cite{(PLOP)douillard2020plop} & 39.11 & 7.81 & 28.75 & 40.48 & 13.61 & 31.59  \\
%           \hline
%           SSUL & 42.03 & 15.80 & 33.35 & 42.10 & 16.02 & 33.46  \\
%           SSUL$\dagger$ & - & - & - & - & - & -  \\
%           %\hline
%           %Joint & 44.30 & 28.20 & 38.90 & 44.30 & 28.20 & 38.90 & 51.10 & 33.25 & 38.90 & 51.10 & 33.25 & 38.90 & 44.30 & 28.20 & 38.90  \\
%           \bottomrule
%         \end{tabular}
%         \end{adjustbox}
%       \end{table}
% \end{minipage} \hfill
% \begin{minipage}[t]{0.5\textwidth}
%   \centering
%     \begin{adjustbox}{max width=\linewidth}
%         \includegraphics{cvpr2021/figures/evolution.png}
%     \end{adjustbox}
%     \captionof{figure}{mIoU evolution on Pascal VOC 2012}
%     \label{fig:miou_evolution}
% \end{minipage}
% \end{table}

% \begin{table}[t]
%     \begin{minipage}[b]{0.4\textwidth}
%       \begin{table}[t]
%         \centering
%         \caption{
%           Experimental results on ADE20K. SSUL$\dagger$ denotes the result using exemplar memory.
%         }
%         \label{tab:sota_ade}
%         \begin{adjustbox}{max width=\linewidth}
%         \begin{tabular}{c||ccc|ccc}
%           \toprule
%           &  \multicolumn{3}{|c}{\textbf{ADE 100-5 (11 tasks)}} & \multicolumn{3}{|c}{\textbf{ADE 100-10 (6 tasks)}}  \\
%           Method & 0-100 & 101-150 & all & 0-100 & 101-150 & all  \\
%           \hline
%           ILT \cite{(ILT)michieli2019incremental} & 0.08 & 1.31 & 0.49 & 0.11 & 3.06 & 1.09  \\
%           MiB \cite{(MiB)cermelli2020modeling} & 36.01 & 5.66 & 25.96 & 38.21 & 11.12 & 29.24  \\
%           PLOP \cite{(PLOP)douillard2020plop} & 39.11 & 7.81 & 28.75 & 40.48 & 13.61 & 31.59  \\
%           \hline
%           SSUL & 42.03 & 15.80 & 33.35 & 42.10 & 16.02 & 33.46  \\
%           SSUL$\dagger$ & - & - & - & - & - & -  \\
%           %\hline
%           %Joint & 44.30 & 28.20 & 38.90 & 44.30 & 28.20 & 38.90 & 51.10 & 33.25 & 38.90 & 51.10 & 33.25 & 38.90 & 44.30 & 28.20 & 38.90  \\
%           \bottomrule
%         \end{tabular}
%         \end{adjustbox}
%       \end{table}
%     \end{minipage} \hfill
%     \begin{minipage}[b]{0.4\textwidth}
%       \begin{table}[t]
%         \centering
%         \caption{
%           Ablation study on VOC 15-1 scenario. pseudo (pseudo labeling); unknown (unknown class modeling with weight transfer); freeze (network freezing); static (static score learning); memory (exemplar memory 100 samples).
%         }
%         \label{tab:ablation}
%           \begin{adjustbox}{max width=0.7\linewidth}
%             \begin{tabular}{ccccc|ccc}
%               \hline
%               & &        &        &        & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}}  \\
%               pseudo & unknown & freeze & static & memory & 0-15 & 16-20 & all \\
%               \hline
%               \hline
%               &                   &  &  &        & 04.32 & 02.36 & 03.86 \\
%               \checkmark &    &     &        &        & 16.73 & 08.43 & 14.76 \\
%               \checkmark & \checkmark &     &        &        & 52.15 & 21.82 & 44.92 \\
%               \checkmark & \checkmark & \checkmark &        &        & 53.02 & 21.62 & 45.54 \\
%               \checkmark & \checkmark & \checkmark & \checkmark &        & 78.06 & 28.54 & 66.27 \\
%               \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 78.92 & 43.86 & 70.58 \\
%               \hline
%               \checkmark &    & \checkmark &        &        & 43.96 & 16.85 & 37.51 \\
%               \checkmark &   & \checkmark & \checkmark &        & 73.42 & 21.79 & 61.12 \\
%               \checkmark & \checkmark &  & \checkmark &  & 53.56 & 14.48 & 44.25 \\
%               \hline
%             \end{tabular}
%           \end{adjustbox}
%       \end{table}
%     \end{minipage}
% \end{table}






% % %------------------------------------------------------------------------------------
% % \begin{table}[t]
% %   \centering
% %   \caption{
% %     Ablation study on PASCAL VOC 2012 dataset. PL (pseudo labeling); unknown (unknown label using saliency maps); freeze (network freezing); sigmoid (change from softmax-CE-loss to sigmoid-CE-loss; memory (replay 100 labels); cutmix (applying cutmix algorithm between current labels and memory labels)
% %   }
% % \label{tab:sota_maskrcnn}

% % \begin{adjustbox}{max width=\linewidth}
% %   \begin{tabular}{cccccc|ccc|ccc|ccc|ccc}
% %     \hline
% %         & &        &     &        &        & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} & \multicolumn{3}{|c}{\textbf{15-5 (2 tasks)}} & \multicolumn{3}{|c}{\textbf{19-1 (2 tasks)}} & \multicolumn{3}{|c}{\textbf{10-1 (11 tasks)}} \\
% %     PL & unknown & freeze & sigmoid & memory & cutmix & 1-15 & 16-20 & all & 1-15 & 16-20 & all & 1-19 & 20 & all & 1-10 & 11-20 & all \\
% %     \hline
% %     \hline
% %     &           &        &     &        &        &  0   &   0   &  0 &  0   &   0   &  0 &  0   &   0   &  0 & 0 & 0 & 0 \\
% %     \checkmark &  &  &     &        &        &  0   &   0   &  0 &  0   &   0   &  0  &  0   &   0   &  0 & 0 & 0 & 0\\
% %     \checkmark &  & \checkmark &     &        &        &  0   &   0   &  0 &  0   &   0   &  0 &  0   &   0   &  0 & 0 & 0 & 0 \\
% %     \hline
% %     \checkmark & \checkmark &  &     &        &        & \emph{32.46} & \emph{5.62} & \emph{26.07} & \emph{64.02} & \emph{38.55} & \emph{57.96} & \emph{72.61} & \emph{13.59} & \emph{69.80} & \emph{15.54} & \emph{21.09} & \emph{9.44} \\
% %     \checkmark & \checkmark &  & \checkmark &        &        & \emph{34.98} & \emph{3.65} & \emph{27.52} & \emph{61.94} & \emph{36.81} & \emph{55.95} & \emph{67.59} & \emph{11.62} & \emph{64.93} & \emph{15.00} & \emph{10.16} & \emph{12.69} \\
% %     \checkmark & \checkmark & \checkmark &     &        &        & \emph{27.10} & \emph{9.91} & \emph{23.01} & \emph{68.51} & \emph{36.03} & \emph{60.77} & \emph{77.15} & \emph{16.62} & \emph{74.27} & \emph{8.25} & \emph{10.72} & \emph{9.42} \\
% %     \checkmark & \checkmark & \checkmark & \checkmark &        &        & \emph{74.90} & \emph{15.71} & \emph{60.81} & \emph{77.42} & \emph{47.16} & \emph{70.21} & \emph{77.09} & \emph{28.69} & \emph{74.78} & \emph{68.29} & \emph{29.96} & \emph{50.04} \\
% %     \hline
% %     \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &        & 76.66 & 29.42 & 65.43 & 78.56 & 50.13 & 71.79 & \emph{77.75} & \emph{39.16} & \emph{75.91} & 0 & 0 & 0 \\
% %     \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 77.09 & 22.61 & 64.12 & 77.79 & 48.74 & 70.87 & 77.16 & 26.04 & 74.73 & 0 & 0 & 0 \\
% %     \checkmark & \checkmark & \checkmark &     & \checkmark &        & 55.49 & 22.43 & 47.62 &  0   &   0   &  0 &  0   &   0   &  0 & 0 & 0 & 0 \\
% %      & \checkmark & \checkmark & \checkmark & \checkmark &  & 77.00 & 29.21 & 65.62 &  &  &  &  &  & & 0 & 0 & 0 \\
% %      \hline
% %      \checkmark & \checkmark & \checkmark & \checkmark &  &  & 59.44 & 16.31 & 49.17 &  &  &  &  &  & & 0 & 0 & 0 \\
% %       & \checkmark & \checkmark & \checkmark &  &  & 60.37 & 14.50 & 49.45 &  &  &  &  &  & & 0 & 0 & 0 \\
% %       \checkmark & \checkmark &  & \checkmark & & & 35.00 & 3.65 & 27.53 &  &  &  &  &  & & 0 & 0 & 0 \\
% %       & \checkmark &  & \checkmark &  &  & 5.47 & 2.11 & 4.67 &  &  &  &  &  & & 0 & 0 & 0 \\
% %       %& \checkmark &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  \\
% %     \hline
% %   \end{tabular}
% %   \end{adjustbox}
% %   \vspace{5mm}

% % \end{table}
% % %------------------------------------------------------------------------------------



% % % %------------------------------------------------------------------------------------
% % % \begin{table}[t]
% % %   \centering
% % %   \caption{
% % %     PASCAL VOC 2012 with 15-5 case. \textbf{Shared backbone}.
% % %     PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map) 
% % %   }
% % % \label{tab:sota_maskrcnn}

% % % \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{cccc|c}
% % %     \hline
% % %     PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %       &  &  &  & 16.20 \\
% % %      \checkmark &  &  &  & 54.03 \\
% % %      \checkmark & \checkmark &  &  & 58.64 \\
% % %      \checkmark &  & \checkmark &  & 59.15 \\
% % %      \checkmark & \checkmark &  & \checkmark & 58.49 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|cccc|c}
% % %     \hline
% % %     Iter & PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 &  &  &  &  & 46.94 \\
% % %     300 &  &  &  &  & 25.95 \\
% % %     500 &  &  &  &  & 19.48 \\
% % %     700 &  &  &  &  & 17.86 \\
% % %     900 &  &  &  &  & 16.20 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|cccc|c}
% % %     \hline
% % %     Iter & PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 & \checkmark &  &  &  & 54.92 \\
% % %     300 & \checkmark &  &  &  & 54.61 \\
% % %     500 & \checkmark &  &  &  & 54.11 \\
% % %     700 & \checkmark &  &  &  & 54.33 \\
% % %     900 & \checkmark &  &  &  & 54.03 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|cccc|c}
% % %     \hline
% % %     Iter & PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 & \checkmark & \checkmark &  &  & 55.33 \\
% % %     300 & \checkmark & \checkmark &  &  & 58.11 \\
% % %     500 & \checkmark & \checkmark &  &  & 57.81 \\
% % %     700 & \checkmark & \checkmark &  &  & 58.62 \\
% % %     900 & \checkmark & \checkmark &  &  & 58.64 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|cccc|c}
% % %     \hline
% % %     Iter & PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 & \checkmark &  & \checkmark &  & 54.93 \\
% % %     300 & \checkmark &  & \checkmark &  & 58.83 \\
% % %     500 & \checkmark &  & \checkmark &  & 57.83 \\
% % %     700 & \checkmark &  & \checkmark &  & 58.87 \\
% % %     900 & \checkmark &  & \checkmark &  & 59.15 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|cccc|c}
% % %     \hline
% % %     Iter & PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 & \checkmark & \checkmark &  & \checkmark & 55.12 \\
% % %     300 & \checkmark & \checkmark &  & \checkmark & 57.99 \\
% % %     500 & \checkmark & \checkmark &  & \checkmark & 57.77 \\
% % %     700 & \checkmark & \checkmark &  & \checkmark & 58.64 \\
% % %     900 & \checkmark & \checkmark &  & \checkmark & 58.49 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|cccc|c}
% % %     \hline
% % %     Iter & PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 &  &  & \checkmark & \checkmark & 54.81 \\
% % %     300 &  &  & \checkmark & \checkmark & 50.89 \\
% % %     500 &  &  & \checkmark & \checkmark & 45.55 \\
% % %     700 &  &  & \checkmark & \checkmark & 47.62 \\
% % %     900 &  &  & \checkmark & \checkmark & 44.90 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
  
  
% % % %   \begin{adjustbox}{max width=\linewidth}
% % % %   \begin{tabular}{c|cccc|c}
% % % %     \hline
% % % %     Iter & PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % % %     \hline
% % % %     100 &  &  &  &  &  \\
% % % %     300 &  &  &  &  &  \\
% % % %     500 &  &  &  &  &  \\
% % % %     700 &  &  &  &  &  \\
% % % %     900 &  &  &  &  &  \\
% % % %     \hline
% % % %   \end{tabular}
% % % %   \end{adjustbox}
% % % %   \vspace{5mm}
  
  
% % % \end{table}
% % % %------------------------------------------------------------------------------------




% % % %------------------------------------------------------------------------------------
% % % \begin{table}[t]
% % %   \centering
% % %   \caption{
% % %     PASCAL VOC 2012 with 15-5 case. \textbf{Fixed prev network}.
% % %     PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map) 
% % %   }
% % % \label{tab:sota_maskrcnn}

% % % \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{cccc|c}
% % %     \hline
% % %     PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %       &  &  &  &  \\
% % %      \checkmark &  &  &  &  \\
% % %      \checkmark & \checkmark &  &  &  \\
% % %      \checkmark &  & \checkmark &  &  \\
% % %      \checkmark & \checkmark &  & \checkmark &  \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|cccc|c}
% % %     \hline
% % %     Iter & PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 & \checkmark &  & \checkmark &  & 59.82 \\
% % %     300 & \checkmark &  & \checkmark &  & 60.24 \\
% % %     500 & \checkmark &  & \checkmark &  & 62.52 \\
% % %     700 & \checkmark &  & \checkmark &  & 62.22 \\
% % %     900 & \checkmark &  & \checkmark &  & 59.68 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|cccc|c}
% % %     \hline
% % %     Iter & PL & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 & \checkmark &  & \checkmark & \checkmark & 60.08 \\
% % %     300 & \checkmark &  & \checkmark & \checkmark & 60.35 \\
% % %     500 & \checkmark &  & \checkmark & \checkmark & 62.63 \\
% % %     700 & \checkmark &  & \checkmark & \checkmark & 62.17 \\
% % %     900 & \checkmark &  & \checkmark & \checkmark & 60.18 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % % \end{table}
% % % %------------------------------------------------------------------------------------




% % % %------------------------------------------------------------------------------------
% % % \begin{table}[t]
% % %   \centering
% % %   \caption{
% % %     PASCAL VOC 2012 with 15-5 case. \textbf{Fixed prev network with unknown label}.
% % %     PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map); Stack
% % %   }
% % % \label{tab:sota_maskrcnn}

% % % \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{ccccc|c}
% % %     \hline
% % %     PL & Stack & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %       &  &  &  &  &  \\
% % %      \checkmark &  &  &  &  &  \\
% % %      \checkmark & &  \checkmark &  &  &  \\
% % %      \checkmark &  &  & \checkmark &  &  \\
% % %      \checkmark & &  \checkmark &  & \checkmark &  \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}

% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|ccccc|c}
% % %     \hline
% % %     Iter & PL & Stack & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 & \checkmark &  &  &  & \checkmark & 59.78 \\
% % %     300 & \checkmark &  &  &  & \checkmark & 63.56 \\
% % %     500 & \checkmark &  &  &  & \checkmark & 63.35 \\
% % %     700 & \checkmark &  &  &  & \checkmark & 63.23 \\
% % %     900 & \checkmark &  &  &  & \checkmark & 63.75 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|ccccc|c}
% % %     \hline
% % %     Iter & PL & Stack & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 & \checkmark & \checkmark &  &  & \checkmark & 65.32 \\
% % %     300 & \checkmark & \checkmark &  &  & \checkmark & 65.20 \\
% % %     500 & \checkmark & \checkmark &  &  & \checkmark & 64.73 \\
% % %     700 & \checkmark & \checkmark &  &  & \checkmark & 64.40 \\
% % %     900 & \checkmark & \checkmark &  &  & \checkmark & 64.37 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
    
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|ccccc|c}
% % %     \hline
% % %     Iter & PL & Stack & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 & \checkmark & \checkmark &  & \checkmark & \checkmark & 65.32 \\
% % %     300 & \checkmark & \checkmark &  & \checkmark & \checkmark & 65.51 \\
% % %     500 & \checkmark & \checkmark &  & \checkmark & \checkmark & 65.00 \\
% % %     700 & \checkmark & \checkmark &  & \checkmark & \checkmark & 64.83 \\
% % %     900 & \checkmark & \checkmark &  & \checkmark & \checkmark & 64.27 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
% % %   \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|ccccc|c}
% % %     \hline
% % %     Iter & PL & Stack & Mem (first) & Mem (last) & Sal  & mIoU (all) \\
% % %     \hline
% % %     100 & \checkmark & \checkmark &  & \checkmark & \checkmark & 56.54 \\
% % %     300 & \checkmark & \checkmark &  & \checkmark & \checkmark & 60.09 \\
% % %     500 & \checkmark & \checkmark &  & \checkmark & \checkmark & 63.08 \\
% % %     700 & \checkmark & \checkmark &  & \checkmark & \checkmark & 65.08 \\
% % %     900 & \checkmark & \checkmark &  & \checkmark & \checkmark & 65.79 \\
% % %     1100 & \checkmark & \checkmark &  & \checkmark & \checkmark & 66.31 \\
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}
  
  
% % % \end{table}
% % % %------------------------------------------------------------------------------------




% % % %------------------------------------------------------------------------------------
% % % \begin{table}[t]
% % %   \centering
% % %   \caption{
% % %     PASCAL VOC 2012 with 15-5 case. PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map); Fix (fixed prev network); Stack; init (head initializer - kaming he normal, mean zero normal)
% % %   }
% % % \label{tab:sota_maskrcnn}

% % % \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{ccccccc|c}
% % %     \hline
% % %     PL & Mem & Sal & Fix & Unknown & Stack & init & mIoU (all) \\
% % %     \hline
% % %       &  &  &  &  &  & he & 16.20 \\
% % %      \checkmark &  &  &  & & &  he & 54.03 \\
% % %      \checkmark & \checkmark &  & & &  &  he & 59.15 \\
% % %      \checkmark & \checkmark & \checkmark &  &  & &  he & 58.49 \\
% % %      - & - & - & - & - & - & - & - \\
% % %      \checkmark & \checkmark &  & \checkmark & &  &  he & 62.22 \\
% % %      \checkmark & \checkmark & \checkmark & \checkmark &  & &  he & 62.17 \\
% % %      - & - & - & - & - & - & - & - \\
% % %      &  & \checkmark & \checkmark &  & &  he &  \\
% % %       & \checkmark & \checkmark & \checkmark &  & &  he & third \\
% % %      - & - & - & - & - & - & - & - \\
% % %      \checkmark &  & \checkmark & \checkmark & \checkmark & &  he & 63.17 \\
% % %      \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  he & 63.44 \\
% % %      \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  he & \\ %64.27 \\
% % %      - & - & - & - & - & - & - & - \\
% % %      \checkmark &  & \checkmark & \checkmark & \checkmark & & zero & left  \\
% % %      \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  zero & 62.14  \\
% % %      \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  zero &  \\ %66.31  \\
     
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}

% % % \end{table}
% % % %------------------------------------------------------------------------------------


% % % %------------------------------------------------------------------------------------
% % % \begin{table}[t]
% % %   \centering
% % %   \caption{
% % %     PASCAL VOC 2012 with 15-5 case. PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map); Fix (fixed prev network); Stack; init (head initializer - kaming he normal, mean zero normal)
% % %   }
% % % \label{tab:sota_maskrcnn}

% % % \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{cccccc|c}
% % %     \hline
% % %     PL & Mem & Sal & Fix & Unknown & Stack  & mIoU (all) \\
% % %     \hline
% % %       &  &  &  &  &  & 16.20 \\
% % %      \checkmark &  &  &  & & & 54.03 \\
% % %      \checkmark & \checkmark &  & & &  & 59.15 \\
% % %      \checkmark & \checkmark & \checkmark &  &  & & 58.49 \\
% % %      \checkmark & \checkmark & \checkmark & \checkmark &  & & 62.17 \\
% % %      \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  &  63.44 \\
% % %      \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  65.00 \\
     
% % %      - & - & - & - & - & - & -  \\
% % %      &  & \checkmark & \checkmark &  & &   \\
% % %       & \checkmark & \checkmark & \checkmark &  & &  third \\
% % %      - & - & - & - & - & - & -  \\
% % %      \checkmark &  & \checkmark & \checkmark & \checkmark & &  63.17 \\
% % %      \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &  63.44 \\
% % %      \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &  \\ %64.27 \\
% % %      - & - & - & - & - & - & -  \\
% % %      \checkmark &  & \checkmark & \checkmark & \checkmark &  & left  \\
% % %      \checkmark &  & \checkmark & \checkmark & \checkmark & \checkmark &   62.14  \\
% % %      \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &   \\ %66.31  \\
     
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}

% % % \end{table}
% % % %------------------------------------------------------------------------------------

% % % %------------------------------------------------------------------------------------
% % % \begin{table}[t]
% % %   \centering
% % %   \caption{
% % %     PASCAL VOC 2012 with 15-5 case. PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map); Fix (fixed prev network); Stack;
% % %   }
% % % \label{tab:sota_maskrcnn}

% % % \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{ccccc|c}
% % %     \hline
% % %     Fix & PL & Sal  & Unknown & Stack  & mIoU (all) \\
% % %     \hline
% % %       &  &  &  &   & 16.20 \\
% % %       & \checkmark &  &  &   & 54.34 \\
% % %       &  & \checkmark &  &   & 25.01 \\
% % %       \hline
% % %      \checkmark &  &  & & & 60.32 \\
% % %      \checkmark &  & \checkmark & &  & 58.50 \\
% % %       \checkmark & \checkmark &  &  &   & 60.21 \\
% % %       \checkmark & \checkmark & \checkmark &  &   & 60.42 \\
% % %      \hline
% % %       \checkmark & \checkmark & \checkmark & \checkmark &   & 63.39  \\
% % %       \checkmark & \checkmark & \checkmark & \checkmark & \checkmark  & 66.61 \\
% % %       \hline
% % %       %\checkmark &  & \checkmark & \checkmark &   & 66.15  \\
% % %       \checkmark &  & \checkmark & \checkmark & \checkmark  & 66.15  \\     
     
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}

% % % \end{table}
% % % %------------------------------------------------------------------------------------



% % % %------------------------------------------------------------------------------------
% % % \begin{table}[t]
% % %   \centering
% % %   \caption{
% % %     PASCAL VOC 2012 with 15-5 case. PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map); Fix (fixed prev network); Stack;
% % %   }
% % % \label{tab:sota_maskrcnn}

% % % \begin{adjustbox}{max width=\linewidth}
% % %   \begin{tabular}{c|cc|ccc}
% % %     \hline
% % %     loss & training stack & testing stack  & mIoU (1-15) & mIoU (16-20) & mIoU (all) \\
% % %     \hline
% % %     CE loss &  &  & & & \\
% % %     CE loss & \checkmark & \checkmark & 69.27 & 48.33 & 65.03  \\
% % %     \hline
% % %     BCE loss &  &  & 71.59 & 35.85 & 63.39 \\
% % %     BCE loss & \checkmark &  & & & 60.58 \\
% % %     BCE loss &  & \checkmark & 71.67 & 48.32 & 66.61 \\
% % %     BCE loss & \checkmark & \checkmark & 71.66 & 43.46 & 65.08  \\
     
% % %     \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \vspace{5mm}

% % % \end{table}
% % % %------------------------------------------------------------------------------------


% % %------------------------------------------------------------------------------------
% % \begin{table}[t]
% %   \centering
% %   \caption{
% %     PASCAL VOC 2012 with 15-5 (2 tasks) case. PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map); Fix (fixed prev network); Stack;
% %   }
% % \label{tab:sota_maskrcnn}

% % \begin{adjustbox}{max width=\linewidth}
% %   \begin{tabular}{c|c|c|cc|cc|ccc|ccc}
% %     \hline
% %     Model & loss & freeze & stack & div & training stack & testing stack & mem & cutmix & batch & 1-15 & 16-20 & all \\
% %     \hline
% %     MB2 & CE loss &   & - & - &  &  & & & 32 & 63.48 & 42.40 & 58.46 \\
% %     MB2 & CE loss &  \checkmark & - & - &  &  & & & 32 &  69.32 & 47.67 & 64.16 \\
% %     \hline
% %     MB2 & CE loss &  \checkmark & feat & 1 &  &  & & & 32 & & & \\
% %     MB2 & CE loss &  \checkmark & feat & 1 &  \checkmark & \checkmark & & & 32 &  67.42 & 44.08 & 61.86  \\
% %     MB2 & CE loss &  \checkmark & feat & 2 &  \checkmark & \checkmark & & & 32 &  68.73 & 46.41 & 63.42  \\
% %     MB2 & CE loss &  \checkmark & feat & 5 &  \checkmark & \checkmark & & & 32 &  69.21 & 47.47 & 64.03  \\
% %     \hline
% %     MB2 & CE loss &  \checkmark & score & 1 &  &  & & & 32 & & &  \\
% %     MB2 & CE loss &  \checkmark & score & 1 &  \checkmark & \checkmark & & & 32 &  69.27 & 48.33 & 65.03  \\
% %     \hline
% %     MB2 & CE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & & & 32 &  69.40 & 47.85 & 64.27  \\
% %     MB2 & CE loss &  \checkmark & score & 2 &  \checkmark & \checkmark & & & 32 &  69.27 & 47.17 & 64.01  \\
% %     MB2 & CE loss &  \checkmark & score & 1 &  \checkmark & \checkmark & & & 32 &   &  &   \\
% %     \hline
% %     \hline
% %     MB2 & BCE loss &   & - & - &   &  & & &  32 & 59.51 & 38.35 & 54.46  \\
% %     MB2 & BCE loss &  \checkmark & - & - &   &  & & &  32 & 71.59 & 35.85 & 63.02 \\
% %     \hline
% %     MB2 & BCE loss &  \checkmark & score & 5 &  \checkmark &  & & & 32 &  71.51 & 27.39 & 61.00 \\
% %     MB2 & BCE loss &  \checkmark & score & 5 &   & \checkmark & & & 32 &  71.32 & 48.83 & 65.97 \\
% %     MB2 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark &  & & 32 & \textbf{71.69} & \textbf{48.25} & \textbf{66.05}  \\
% %     MB2 & BCE loss &   & score & 5 &  \checkmark & \checkmark &  & & 32 & 59.83 & 38.26 & 54.72  \\
    
% %     \hline
% %     MB2 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark &  & & 32 & \textbf{71.69} & \textbf{48.25} & \textbf{66.05}  \\
% %     MB2 & BCE loss &  \checkmark & score & 2 &  \checkmark & \checkmark &  & & 32 & 71.70 & 46.98 & 65.76  \\
% %     MB2 & BCE loss &  \checkmark & score & 1 &  \checkmark & \checkmark &  & & 32 & 71.67 & 43.24 & 64.84  \\
% %     \hline
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark &     &  & 32 & 78.07 & 45.18 & 70.02 \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 &  & 64 & \textbf{78.25} & \textbf{47.97} & \textbf{71.03} \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 & \checkmark (1.0) & 32 & 77.76 & 45.95 & 70.19 \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 & \checkmark (0.5) & 32 & 78.13 & 46.47 & 70.60 \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 & \checkmark (0.5) & 64 & 78.17 & 47.66 & 70.90 \\
% %     \hline
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 & \checkmark (0.5) & 32 & 78.13 & 46.47 & 70.60 \\
% %     R101 & BCE loss &  \checkmark & score & 7 &  \checkmark & \checkmark & 100 & \checkmark (0.5) & 32 & 78.11 & 46.42 & 70.57 \\
% %     R101 & BCE loss &  \checkmark & score & 10 &  \checkmark & \checkmark & 100 & \checkmark (0.5) & 32 & 78.08 & 46.38 & 70.54 \\
% %     \hline
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 &  & 64 & \textbf{78.78} & \textbf{47.76} & \textbf{71.39} \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 50 &  & 64 & 78.90 & 48.26 & 71.61 \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 20 &  & 64 & 78.46 & 47.20 & 71.02 \\
    
% %     \hline
% %   \end{tabular}
% %   \end{adjustbox}
% %   \vspace{5mm}

% % \end{table}
% % %------------------------------------------------------------------------------------




% % %------------------------------------------------------------------------------------
% % \begin{table}[t]
% %   \centering
% %   \caption{
% %     PASCAL VOC 2012 with 15-1 (6 tasks) case. PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map); Fix (fixed prev network); Stack;
% %   }
% % \label{tab:sota_maskrcnn}

% % \begin{adjustbox}{max width=\linewidth}
% %   \begin{tabular}{c|c|c|cc|cc|ccc|ccc}
% %     \hline
% %     Model & loss & freeze & stack & div & training stack & testing stack & mem & cutmix & batch & 1-15 & 16-20 & all \\
% %     \hline
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark &  & & 64 & 70.37 & 18.57 & 56.33  \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 (1.0) & & 64 & 77.99 & 37.10 & 68.26  \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 (0.5) & & 64 & 77.22 & 29.10 & 65.76  \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 (1.0) & \checkmark (ori) & 64 &  &  & 64.17  \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 (0.5) & \checkmark (ori) & 64 & 77.29 & 31.28 & 66.39  \\
% %     \hline
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 (1.0) & & 64 & 77.99 & 37.10 & 68.26  \\
% %     R101 & BCE loss &  \checkmark & score & 5 &   &  & 100 (1.0) & & 64 & 74.52 & 28.19 & 63.49  \\
% %     \hline
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 (0.5) & \checkmark (ori) & 64 & 76.79 & 27.69 & 65.10  \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 (0.5) & \checkmark (new) & 64 & 74.44 & 22.58 & 62.09  \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 (0.5) & \checkmark (blob) & 64 & 74.41 & 22.49 & 62.05  \\
% %     \hline
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 (0.5) & \checkmark (blob) & 64 & 74.41 & 22.49 & 62.05  \\
% %     R101 & BCE loss &   & score & 5 &  \checkmark & \checkmark & 100 (0.5) & \checkmark (blob) & 64 & 58.58 & 11.78 & 47.44  \\
% %     R101 & BCE loss &   & score & 5 &  \checkmark & \checkmark & 100 (0.5) & \checkmark (blob) & 64 & 65.13 & 04.88 & 50.78  \\
    
% %     \hline
% %   \end{tabular}
% %   \end{adjustbox}
% %   \vspace{5mm}

% % \end{table}
% % %------------------------------------------------------------------------------------



% % %------------------------------------------------------------------------------------
% % \begin{table}[t]
% %   \centering
% %   \caption{
% %     PASCAL VOC 2012 with 19-1 (6 tasks) case. PL (Pseudo Labeling); Mem (Memory); Sal (Saliency map); Fix (fixed prev network); Stack;
% %   }
% % \label{tab:sota_maskrcnn}

% % \begin{adjustbox}{max width=\linewidth}
% %   \begin{tabular}{c|c|c|cc|cc|ccc|ccc}
% %     \hline
% %     Model & loss & freeze & stack & div & training stack & testing stack & mem & cutmix & batch & 1-15 & 16-20 & all \\
% %     \hline
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 100 (1.0) &  & 64 & 76.84 & 30.42 & 74.63  \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 50 (1.0) &  & 64 & 76.55 & 29.04 & 74.29  \\
% %     R101 & BCE loss &  \checkmark & score & 5 &  \checkmark & \checkmark & 20 (1.0) &  & 64 & 76.49 & 29.05 & 74.23  \\
    
% %     \hline
% %   \end{tabular}
% %   \end{adjustbox}
% %   \vspace{5mm}

% % \end{table}
% % %------------------------------------------------------------------------------------



% % %------------------------------------------------------------------------------------
% % \begin{table}[t]
% %   \centering
% %   \caption{
% %     Ablation study on PASCAL VOC 2012 dataset. PL (pseudo labeling); unknown (unknown label using saliency maps); freeze (network freezing); sigmoid (change from softmax-CE-loss to sigmoid-CE-loss; memory (replay 100 labels); cutmix (applying cutmix algorithm between current labels and memory labels)
% %   }
% % \label{tab:sota_maskrcnn}

% % \begin{adjustbox}{max width=\linewidth}
% %   \begin{tabular}{c|cc|ccc|ccc|ccc}
% %     \hline
% %     \textbf{PL}&    \multicolumn{2}{c}{\textbf{Freeze}} & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} & \multicolumn{3}{|c}{\textbf{15-5 (2 tasks)}} & \multicolumn{3}{|c}{\textbf{19-1 (2 tasks)}} \\
% %      & unknown & background & 1-15 & 16-20 & all & 1-15 & 16-20 & all & 1-19 & 20 & all \\
% %     \hline
% %     %\checkmark &            &            & 75.07 & 26.48 & 63.50 &  0   &   0   &  0 &  0   &   0   &  0  \\
% %     %\checkmark &            & \checkmark & 76.66 & 29.42 & 65.43 & 78.56 & 50.13 & 71.79 & 77.11 & 41.57 & 75.42  \\
% %     %\checkmark & \checkmark & \checkmark & 77.99 & 38.82 & 68.67 & 78.77 & 47.00 & 71.20 & 76.85 & 40.42 & 75.12  \\
% %     \checkmark &            &            &  &  &  &  &  &  & 76.88 & 23.13 & 74.32  \\
% %     \checkmark &            & \checkmark &  &  &  &  &  &  & 77.09 & 28.69 & 74.78  \\
% %     \checkmark & \checkmark & \checkmark &  &  &  &  &  &  &  &  &   \\
% %     \hline
% %      &            &            &  &  &  &  &  &  & 69.60 & 18.77 & 67.18  \\
% %      &            & \checkmark &  &  &  &  &  &  &  &  &   \\
% %      & \checkmark & \checkmark &  &  &  &  &  &  &  &  &   \\
% %     \hline
% %   \end{tabular}
% %   \end{adjustbox}
% %   \vspace{5mm}

% % \end{table}
% % %------------------------------------------------------------------------------------


% % %%%%%


% % %------------------------------------------------------------------------------------
% % \begin{table}[t]
% %   \centering
% %   \caption{
% %     Ablation study on PASCAL VOC 2012 dataset. PL (pseudo labeling); unknown (unknown label using saliency maps); freeze (network freezing); sigmoid (change from softmax-CE-loss to sigmoid-CE-loss; memory (replay 100 labels); cutmix (applying cutmix algorithm between current labels and memory labels)
% %   }
% % \label{tab:sota_maskrcnn}

% % \begin{adjustbox}{max width=\linewidth}
% %   \begin{tabular}{cccccc|ccc|ccc|ccc|ccc}
% %     \hline
% %         & &        &     &        &        & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} & \multicolumn{3}{|c}{\textbf{15-5 (2 tasks)}} & \multicolumn{3}{|c}{\textbf{19-1 (2 tasks)}} & \multicolumn{3}{|c}{\textbf{10-1 (11 tasks)}} \\
% %     PL & unknown & freeze & sigmoid & memory & cutmix & 1-15 & 16-20 & all & 1-15 & 16-20 & all & 1-19 & 20 & all & 1-10 & 11-20 & all \\
% %     \hline
% %     \hline
% %     &           &        &     &        &        &  0   &   0   &  0 &  0   &   0   &  0 &  0   &   0   &  0 & 0 & 0 & 0 \\
% %     \checkmark &  &  &     &        &        &  0   &   0   &  0 &  0   &   0   &  0  &  0   &   0   &  0 & 0 & 0 & 0\\
% %     \checkmark &  & \checkmark &     &        &        &  0   &   0   &  0 &  0   &   0   &  0 &  0   &   0   &  0 & 0 & 0 & 0 \\
% %     \hline
% %     \checkmark & \checkmark &  &     &        &        &  32.46  &  5.62  &  26.07  &  64.02  &  38.55  &  57.96  &  72.61  &  13.59  &  69.80  &  15.54  &  21.09  &  9.44  \\
% %     \checkmark & \checkmark &  & \checkmark &        &        &  34.98  &  3.65  &  27.52  &  61.94  &  36.81  &  55.95  &  67.59  &  11.62  &  64.93  &  15.00  &  10.16  &  12.69  \\
% %     \checkmark & \checkmark & \checkmark &     &        &        &  27.10  &  9.91  &  23.01  &  68.51  &  36.03  &  60.77  &  77.15  &  16.62  &  74.27  &  8.25  &  10.72  &  9.42  \\
% %     \checkmark & \checkmark & \checkmark & \checkmark &        &        &  74.90  &  15.71  &  60.81  &  77.42  &  47.16  &  70.21  &  77.09  &  28.69  &  74.78  &  68.29  &  29.96  &  50.04  \\
% %     \hline
% %     \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &        & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% %     \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% %     \checkmark & \checkmark & \checkmark &     & \checkmark &        & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% %      & \checkmark & \checkmark & \checkmark & \checkmark &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & & 0 & 0 & 0 \\
% %      \hline
% %      \checkmark & \checkmark & \checkmark & \checkmark &  &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% %       & \checkmark & \checkmark & \checkmark &  &  & 0 & 0 & 0 & 0 & 0 & 0 & 00 & 0 & 0 & 0 & 0 & 0 \\
% %       \checkmark & \checkmark &  & \checkmark & & & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% %       & \checkmark &  & \checkmark &  &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
% %       %& \checkmark &  & \checkmark &  &  &  &  &  &  &  &  &  &  &  \\
% %     \hline
% %   \end{tabular}
% %   \end{adjustbox}
% %   \vspace{5mm}

% % \end{table}
% % %------------------------------------------------------------------------------------



% % %------------------------------------------------------------------------------------
% % \begin{table}[t]
% %   \centering
% %   \caption{
% %     Ablation study on PASCAL VOC 2012 dataset. PL (pseudo labeling); unknown (unknown label using saliency maps); freeze (network freezing); sigmoid (change from softmax-CE-loss to sigmoid-CE-loss; memory (replay 100 labels); cutmix (applying cutmix algorithm between current labels and memory labels)
% %   }
% % \label{tab:sota_maskrcnn}

% % \begin{adjustbox}{max width=\linewidth}
% %   \begin{tabular}{c|cc|ccc|ccc|ccc}
% %     \hline
% %     \textbf{PL}&    \multicolumn{2}{c}{\textbf{Freeze}} & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} & \multicolumn{3}{|c}{\textbf{15-5 (2 tasks)}} & \multicolumn{3}{|c}{\textbf{19-1 (2 tasks)}} \\
% %      & unknown & background & 1-15 & 16-20 & all & 1-15 & 16-20 & all & 1-19 & 20 & all \\
% %     \hline
% %     %\checkmark &            &            & 75.07 & 26.48 & 63.50 &  0   &   0   &  0 &  0   &   0   &  0  \\
% %     %\checkmark &            & \checkmark & 76.66 & 29.42 & 65.43 & 78.56 & 50.13 & 71.79 & 77.11 & 41.57 & 75.42  \\
% %     %\checkmark & \checkmark & \checkmark & 77.99 & 38.82 & 68.67 & 78.77 & 47.00 & 71.20 & 76.85 & 40.42 & 75.12  \\
% %     \checkmark &            &            &  &  &  &  &  &  & 76.88 & 23.13 & 74.32  \\
% %     \checkmark &            & \checkmark &  &  &  &  &  &  & 77.09 & 28.69 & 74.78  \\
% %     \checkmark & \checkmark & \checkmark &  &  &  &  &  &  &  &  &   \\
% %     \hline
% %      &            &            &  &  &  &  &  &  & 69.60 & 18.77 & 67.18  \\
% %      &            & \checkmark &  &  &  &  &  &  &  &  &   \\
% %      & \checkmark & \checkmark &  &  &  &  &  &  &  &  &   \\
% %     \hline
% %   \end{tabular}
% %   \end{adjustbox}
% %   \vspace{5mm}

% % \end{table}
% % %------------------------------------------------------------------------------------



% % %------------------------------------------------------------------------------------
% % \begin{table}[t]
% %   \centering
% %   \caption{
% %     Ablation study
% %   }
% % \label{tab:sota_maskrcnn}

% % \begin{adjustbox}{max width=\linewidth}
% %   \begin{tabular}{cc|ccc}
% %     \hline
% %      & & \multicolumn{3}{|c}{\textbf{15-1 (6 tasks)}} \\
% %     Unknown Initial & BN Freeze & 1-15 & 16-20 & all \\
% %     \hline
% %     \checkmark &  & 75.77 & 19.06 & 62.27 \\
% %      & \checkmark & 74.21 & 18.06 & 60.84 \\
% %     \checkmark & \checkmark & 77.69 & 23.63 & 64.82 \\
% %     \hline
% %   \end{tabular}
% %   \end{adjustbox}
% %   \vspace{5mm}

% % \end{table}
% % %------------------------------------------------------------------------------------

